LLM-SR: Scientific Equation Discovery via Programming with Large Language Models

Mathematical equations have been unreasonably effective in describing complex natural phenomena across various scientific disciplines. However, discovering such insightful equations from data presents significant challenges due to the necessity of navigating extremely large combinatorial hypothesis spaces. Current methods of equation discovery, commonly known as symbolic regression techniques, largely focus on extracting equations from data alone, often neglecting the domain-specific prior knowledge that scientists typically depend on. They also employ limited representations such as expression trees, constraining the search space and expressiveness of equations. To bridge this gap, we introduce LLM-SR, a novel approach that leverages the extensive scientific knowledge and robust code generation capabilities of Large Language Models (LLMs) to discover scientific equations from data. Specifically, LLM-SR treats equations as programs with mathematical operators and combines LLMs' scientific priors with evolutionary search over equation programs. The LLM iteratively proposes new equation skeleton hypotheses, drawing from its domain knowledge, which are then optimized against data to estimate parameters. We evaluate LLM-SR on four benchmark problems across diverse scientific domains (e.g., physics, biology), which we carefully designed to simulate the discovery process and prevent LLM recitation. Our results demonstrate that LLM-SR discovers physically accurate equations that significantly outperform state-of-the-art symbolic regression baselines, particularly in out-of-domain test settings. We also show that LLM-SR's incorporation of scientific priors enables more efficient equation space exploration than the baselines. Code and data are available: https://github.com/deep-symbolic-mathematics/LLM-SR

==> fig_table_tex/best-score-curve.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.5\linewidth]{fig_table_file/best-score-osc2-all.png}
\caption{\small The \modelname framework
\vspace{-0.5em}
}
\vspace{-0.5em}
\label{fig:best-curve}
\end{figure}

==> fig_table_tex/best-score-pysr.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{fig_table_file/bestscore-osc2-pysr.png}
\caption{\small The \modelname framework
\vspace{-0.5em}
}
\vspace{-0.5em}
\label{fig:best-curve}
\end{figure}

==> fig_table_tex/crossmut-alg.tex <==


\begin{figure}[t]
% \begin{wrapfigure}[20]{r}{0.45\linewidth}
% \vspace{-1.5em}
\centering
\begin{minipage}{0.55\linewidth}
\begin{algorithm}[H]
\fontsize{9}{9}\selectfont
\SetAlgoLined
\SetKwInOut{Require}{Require}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{KwDownTo}{downto}
\SetKw{KwAnd}{and}
\SetKw{KwContinue}{continue}
\caption{$\text{CrossMut}(\pi_\theta, \mathcal{P}, n, m, k)$}
\Input{LLM $\pi_{\theta}$,  database of (program, score) pairs $\mathcal{P}$ , $n$ in-context examples, $m$ samplers, $k$ samples per prompt}
$\mathcal{F} \gets \emptyset$\\
$i \gets 0$\\
\While{$i < m$}{
\textcolor{gray}{\# Sample in-context examples from database}\\
$E \gets \{x_j\}_{j=1}^n$, $x_j \sim \text{SampleDB}(\mathcal{P})$\\
\textcolor{gray}{\# Prompt with new examples}\\
$p \gets \text{MakeFewShotPrompt}(E)$\\
\textcolor{gray}{\# Sample from LLM}\\
$\mathcal{F}_i \gets \{f_j\}_{j=1}^k$, $f_j \sim \pi_\theta(\cdot | p)$\\
\textcolor{gray}{\# Augment outputs}\\
$\mathcal{F} \gets \mathcal{F} + \mathcal{F}_i$\\
$i \gets i + 1$
}
\Output{$\mathcal{F}$}
% Return $\mathcal{F}$
\end{algorithm}
\end{minipage}
\end{figure}
% \end{wrapfigure}

==> fig_table_tex/fig_feynI1211_qual.tex <==


\begin{figure}[t]
\centering
\includegraphics[width=0.6\linewidth]{fig_table_file/feyn_prompts3.pdf}
% {fig_table_file/qual_feyn_I12_11_v3.jpg}
\caption{\small An example of LLM response to Feynman I.12.11 problem, demonstrating model memorization without iterative search.
}
\vspace{-0.5em}
\label{fig:qual-feynI1211}
\vspace{-0.5em}
\end{figure}

==> fig_table_tex/fig_feynI262_qual.tex <==


\begin{figure}[t]
\centering
\includegraphics[width=0.6\linewidth]{fig_table_file/feyn_prompts2.pdf}
% {fig_table_file/qual_feyn_I26_2_v3.jpg}
\caption{\small An example of LLM response to Feynman I.26.2 problem, demonstrating model memorization without iterative search.
}
\vspace{-0.5em}
\label{fig:qual-feynI262}
\vspace{-0.5em}
\end{figure}

==> fig_table_tex/llmsr-alg.tex <==

\begin{figure}[t]
\centering
\begin{minipage}{0.6\linewidth}
% \begin{wrapfigure}[20]{r}{0.55\linewidth}
% \vspace{-1.5em}
% \begin{minipage}{\linewidth}
\begin{algorithm}[H]
\fontsize{9}{9}\selectfont
\SetAlgoLined
\SetKwInOut{Require}{Require}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{KwDownTo}{downto}
\SetKw{KwAnd}{and}
\SetKw{KwContinue}{continue}
\caption{LLM-SR: LLM-guided Equation Discovery}
\Input{LLM $\pi_{\theta}$, dataset $\mathcal{D}$, scientific problem $\mathcal{T}$, 
% \\
$T$ iterations, $n$ in-context examples, 
% \\
$m$ samplers, $k$ samples per prompt}
\BlankLine
% {\textcolor{gray}{\# Initialize database}}\\
% {$\mathcal{B} \gets \emptyset$}\\
{\textcolor{gray}{\# Initialize population}}\\
{$\mathcal{P} \gets \text{InitPop}()$}\\
\For{$t \gets 0$ \KwTo $T-1$}{
{\textcolor{gray}{\# Sample from LLM}}\\
{$\mathcal{F} \gets \text{CrossMut}(\pi_\theta, \mathcal{P}, n, m, k)$}\\
{\textcolor{gray}{\# Execute evaluation function}}\\
% $\mathcal{F}_\text{Evaled} \gets \text{FilterEval}(\mathcal{F},  \mathcal{D})$\\
$\mathcal{P} \gets \mathcal{P} \cup \{(f, s) : f \in \mathcal{F}, s = \text{Eval}_{\mathcal{T}}(f, \mathcal{D})\}$ \\
% $\mathcal{G} \gets \mathcal{G} + \mathcal{C}_\text{Evaled}$\\
\If{$t < T - 1$}{
{\textcolor{gray}{\# Sample from database}}\\
$\mathcal{P} \gets \text{SampleDB}(\mathcal{P},n)$
}
$t \gets t + 1$
}
\Output{$\text{SampleDB}(\mathcal{P},n)$} 
\end{algorithm}
\end{minipage}
% }}
\end{figure}
% \end{wrapfigure}
% \hfill


==> fig_table_tex/spec_code.tex <==
\begin{figure}[!t]
{\small
\begin{minted}[
frame=lines,
framesep=2mm,
baselinestretch=1.,
fontsize=\footnotesize
]{python}
"""
Find the mathematical function skeleton that represents E. Coli bacterial growth rate, given data on the population density of bacterial species, substrate concentration, temperature, and pH level.
"""

import numpy as np
from scipy.optimize import minimize

def loss_function(params, x0, x1, x2, x3, y_true):
    y_pred = equation(x0, x1, x2, x3, params)
    return np.mean((y_pred - y_true) ** 2)

def evaluate(data: dict) -> float:
    """Evaluate equation on input and output observations."""
    # Load true data observations
    inputs, outputs = data['inputs'], data['outputs']
    # Optimize equation skeleton parameters
    loss_partial = lambda params: loss_function(params, *inputs.T[:4], outputs)
    params_initial_guess = [1.0]*P
    result = minimize(loss_partial, params_initial_guess, method='BFGS')
    optimized_params = result.x
    # Return evaluation score
    score = loss_function(optimized_params, *inputs.T[:4])
    return -score if not np.isnan(score) and not np.isinf(score) else None

def equation_v0(x0: np.ndarray, x1: np.ndarray, x2: np.ndarray, 
x3: np.ndarray, params: np.ndarray) -> np.ndarray:
    """Find mathematical function skeleton for the bacterial growth rate.
    Args:
        x0: Population density of the bacterial species.
        x1: Substrate concentration.
        x2: Temperature.
        x3: pH level.
        params: Array of numeric parameters to be optimized
    Return:
        A numpy array representing bacterial growth rate
    """
    return params[0]*x0 + params[1]*x1 + params[2]*x2 + params[3]*x3 + params[4]

def equation_v1(x0: np.ndarray, x1: np.ndarray, x2: np.ndarray, 
x3: np.ndarray, params: np.ndarray) -> np.ndarray:
    """Improved version of equation_v0"""
\end{minted}
}
\caption{Python code for finding the mathematical function skeleton.}
\label{fig:code}
\end{figure}



% """
% Find the mathematical function skeleton that represents E. Coli bacterial growth rate, given data on the population density of bacterial species, substrate concentration, temperature, and pH level.
% """

% import numpy as np
% from scipy.optimize import minimize

% def loss_function(params, x0, x1, x2, x3, y_true):
%     y_pred = equation(x0, x1, x2, x3, params)
%     return np.mean((y_pred - y_true) ** 2)

% def evaluate(data: dict) -> float:
%     """Evaluate equation on true inputs and outputs observations."""
%     inputs, outputs = data['inputs_train'], data['outputs_train']
%     # Optimize model parameters
%     loss_partial = lambda params: loss_function(params, *inputs.T[:4], outputs)
%     params_initial_guess = [1.0]*P
%     result = minimize(loss_partial, params_initial_guess, method='BFGS')
%     if np.isnan(loss) or np.isinf(loss): return None
%     # Return validation score
%     inputs_val, outputs_val = data['inputs_val'], data['outputs_val']
%     feedback = loss_function(optimized_params, *inputs_val.T[:4])
%     return -feedback if not np.isnan(feedback) and not np.isinf(feedback) else None

% def equation(x0: np.ndarray, x1: np.ndarray, x2: np.ndarray, 
% x3: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """Find mathematical function skeleton for the bacterial growth rate.
%     Args:
%         x0: Population density of the bacterial species.
%         x1: Substrate concentration.
%         x2: Temperature.
%         x3: pH level.
%         params: Array of numeric parameters to be optimized
%     Return:
%         A numpy array representing bacterial growth rate
%     """
%     return params[0]*x0 + params[1]*x1 + params[2]*x2 + params[3]*x3 + params[4]






==> fig_table_tex/spec_feyn.tex <==
\begin{figure}[!t]
{\small
\begin{minted}[
frame=lines,
framesep=2mm,
baselinestretch=1.,
fontsize=\footnotesize
]{python}
% """
% Find the mathematical function structure that represents the resultant intensity due to the interference of two coherent light sources.
% """

% import numpy as np
% from scipy.optimize import minimize

% def loss_function(params, x0, x1, x2, y_true):
%     y_pred = equation(x0, x1, x2, params)
%     return np.mean((y_pred - y_true) ** 2)

% def evaluate(data: dict) -> float:
%     """Evaluate equation on input and output observations."""
%     # Load true data observations
%     inputs, outputs = data['inputs'], data['outputs']
%     # Optimize equation skeleton parameters
%     loss_partial = lambda params: loss_function(params, *inputs.T[:3], outputs)
%     params_initial_guess = [1.0]*P
%     result = minimize(loss_partial, params_initial_guess, method='BFGS')
%     optimized_params = result.x
%     # Return evaluation score
%     score = loss_function(optimized_params, *inputs.T[:3])
%     return -score if not np.isnan(score) and not np.isinf(score) else None

% def equation_v0(x0: np.ndarray, x1: np.ndarray, x2: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """Find mathematical function for the resultant intensity due to interference of two waves given their individual intensities and the phase difference between them.
%     Args:
%         x0: A numpy array representing the intensity of the first wave.
%         x1:A numpy array representing the intensity of the second wave.
%         x2: A numpy array representing the phase difference between the two waves.
%         params: Array of numeric parameters to be optimized
%     Return:
%         A numpy array with the calculated resultant intensity.
%     """
%     return params[0]*x0 + params[1]*x1 + params[2]*x2 + params[3]

% def equation_v1(x0: np.ndarray, x1: np.ndarray, x2: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """Improved version of equation_v0"""
\end{minted}
}
\caption{Python code for finding the mathematical function skeleton.}
\label{fig:code}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%Feyn I-37-4 Prompt:
% Can you give me the complete version of last function?

% Consider the physical meaning and relationships of inputs when completing the function.

% """
% Find the mathematical function structure that represents the resultant intensity due to the interference of two coherent light sources.
% """

% import numpy as np
% from scipy.optimize import minimize

% def loss_function(params, x0, x1, x2, y_true):
%     y_pred = equation(x0, x1, x2, params)
%     return np.mean((y_pred - y_true) ** 2)

% def evaluate(data: dict) -> float:
%     """Evaluate equation on input and output observations."""
%     # Load true data observations
%     inputs, outputs = data['inputs'], data['outputs']
%     # Optimize equation skeleton parameters
%     loss_partial = lambda params: loss_function(params, *inputs.T[:3], outputs)
%     params_initial_guess = [1.0]*P
%     result = minimize(loss_partial, params_initial_guess, method='BFGS')
%     optimized_params = result.x
%     # Return evaluation score
%     score = loss_function(optimized_params, *inputs.T[:3])
%     return -score if not np.isnan(score) and not np.isinf(score) else None

% def equation_v0(x0: np.ndarray, x1: np.ndarray, x2: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """Find mathematical function for the resultant intensity due to interference of two waves given their individual intensities and the phase difference between them.
%     Args:
%         x0: intensity of the first wave.
%         x1: intensity of the second wave.
%         x2: phase difference between the two waves.
%         params: Array of numeric parameters to be optimized
%     Return:
%         A numpy array with the calculated resultant intensity.
%     """
%     return params[0]*x0 + params[1]*x1 + params[2]*x2 + params[3]

% def equation_v1(x0: np.ndarray, x1: np.ndarray, x2: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """Improved version of equation_v0"""
%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%
%Feyn I-37-4 Response:
% def equation(x0: np.ndarray, x1: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """
%     Find mathematical function for the angle of refraction given the refractive index and the angle of incidence.
    
%     Args:
%         x0: A numpy array representing the refractive index of the medium.
%         x1: A numpy array representing the angle of incidence.
%         params: Array of model numeric constants or parameters to be optimized. 
        
%     Returns:
%         A numpy array with the calculated angle of refraction.
%     """
%     return params[0] * np.arcsin(params[1] * n * np.sin(theta2))
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%Feyn I-26-2 Prompt:
% """
% Find the mathematical function structure that represents the relationship between the angle of incidence and the angle of refraction.
% """
% import numpy as np
% from scipy.optimize import minimize

% def loss_function(params, x0, x1, y_true):
%     y_pred = equation(x0, x1, params)
%     return np.mean((y_pred - y_true) ** 2)

% def evaluate(data: dict) -> float:
%     """Evaluate equation on input and output observations."""
%     # Load true data observations
%     inputs, outputs = data['inputs'], data['outputs']
%     # Optimize equation skeleton parameters
%     loss_partial = lambda params: loss_function(params, *inputs.T[:2], outputs)
%     params_initial_guess = [1.0]*P
%     result = minimize(loss_partial, params_initial_guess, method='BFGS')
%     optimized_params = result.x
%     # Return evaluation score
%     score = loss_function(optimized_params, *inputs.T[:2])
%     return -score if not np.isnan(score) and not np.isinf(score) else None

% def equation_v0(x0: np.ndarray, x1: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """
%     Find mathematical function for the angle of refraction given the refractive index and the angle of incidence.
    
%     Args:
%         x0: A numpy array representing the refractive index of the medium.
%         x1: A numpy array representing the angle of incidence.
%         params: Array of model numeric constants or parameters to be optimized. 
        
%     Returns:
%         A numpy array with the calculated angle of refraction.
%     """
%     theta1 = params[0]*x0 + params[1]*x2 + params[3]
%     return theta1

% def equation_v1(x0: np.ndarray, x1: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """Improved version of equation_v0"""
%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%
%%Feyn I-26-2 Response:
% def equation(x0: np.ndarray, x1: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """
%     Find mathematical function for the angle of refraction given the refractive index and the angle of incidence.
    
%     Args:
%         x0: A numpy array representing the refractive index of the medium.
%         x1: A numpy array representing the angle of incidence.
%         params: Array of model numeric constants or parameters to be optimized. 
        
%     Returns:
%         A numpy array with the calculated angle of refraction.
%     """
%     return params[0] * np.arcsin(params[1] * n * np.sin(theta2))
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%Feyn I-12-11 Prompt:
% """
% Find the mathematical function structure that represents the force on a charge due to electric and magnetic fields.
% """
% import numpy as np
% from scipy.optimize import minimize

% def loss_function(params, x0, x1, x2, x3, x4, y_true):
%     y_pred = equation(x0, x1, x2, x3, x4, params)
%     return np.mean((y_pred - y_true) ** 2)

% def evaluate(data: dict) -> float:
%     """Evaluate equation on input and output observations."""
%     # Load true data observations
%     inputs, outputs = data['inputs'], data['outputs']
%     # Optimize equation skeleton parameters
%     loss_partial = lambda params: loss_function(params, *inputs.T[:5], outputs)
%     params_initial_guess = [1.0]*P
%     result = minimize(loss_partial, params_initial_guess, method='BFGS')
%     optimized_params = result.x
%     # Return evaluation score
%     score = loss_function(optimized_params, *inputs.T[:5])
%     return -score if not np.isnan(score) and not np.isinf(score) else None

% def equation_v0(x0: np.ndarray, x1: np.ndarray, x2: np.ndarray, x3: np.ndarray, x4: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """
%     Find mathematical function for force given a charge, electric field, magnetic field, velocity of the charge, and the angle between velocity and magnetic field.
    
%     Args:
%         x0: A numpy array representing the charge.
%         x1: A numpy array representing the electric field.
%         x2: A numpy array representing the magnetic field.
%         x3: A numpy array representing the velocity of the charge.
%         x4: A numpy array representing the angle between velocity and magnetic field direction.
%         params: Array of model numeric constants or parameters to be optimized.
        
%     Returns:
%         A numpy array with the calculated force.
%     """
%     return params[0]*x0 + params[1]*x1 + params[2]*x2 + params[3]*x3 + params[4]*x4 + params[5]

% def equation_v1(x0: np.ndarray, x1: np.ndarray, x2: np.ndarray, x3: np.ndarray, x4: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """Improved version of equation_v0"""
%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%
%%Feyn I-12-11 Response:
% def equation(x0: np.ndarray, x1: np.ndarray, params: np.ndarray) -> np.ndarray:
%     """
%     Find mathematical function for the angle of refraction given the refractive index and the angle of incidence.
    
%     Args:
%         x0: A numpy array representing the refractive index of the medium.
%         x1: A numpy array representing the angle of incidence.
%         params: Array of model numeric constants or parameters to be optimized. 
        
%     Returns:
%         A numpy array with the calculated angle of refraction.
%     """
%     return params[0] * np.arcsin(params[1] * x0 * np.sin(x1)) + params[2]
%%%%%%%%%%%%%%%%%%%%%

==> fig_table_tex/table_feyn_ppl.tex <==


% \begin{table}[tbp]
\begin{wraptable}[9]{r}{0.5\linewidth}
\centering
\vspace{-1.5em}
\resizebox{\linewidth}{!}{
\begin{tabular}{lc}
\toprule
Benchmark Problem & PPL (\texttt{Mixtral})\\
 % & man (std) \\
\midrule
AI Feynman \cite{AI-Feynman-Science-2020} & 3.1 (std: 0.895) \\
Oscillation 1 & 6.24 \\
Oscillation 2 & 5.27 \\
E. coli Growth & 6.93 \\
\bottomrule
\end{tabular}
}
\caption{Perplexity of equations for $120$ Feynman benchmark problems compared to our new benchmarks with custom models on \texttt{Mixtral} model.}
\label{table_perplexity}
\end{wraptable}
% \end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

